LLaSA: A Sensor-Aware LLM for Natural Language Reasoning of Human Activity from IMU Data

Wearable systems can recognize activities from IMU data but often fail to explain their underlying causes or contextual significance. To address this limitation, we introduce two large-scale resources: SensorCap, comprising 35,960 IMU--caption pairs, and OpenSQA, with 199,701 question--answer pairs designed for causal and explanatory reasoning. OpenSQA includes a curated tuning split (Tune-OpenSQA) optimized for scientific accuracy, narrative clarity, and diagnostic insight. Leveraging these datasets, we develop LLaSA (Large Language and Sensor Assistant), a family of compact sensor-aware language models (7B and 13B) that generate interpretable, context-rich responses to open-ended questions grounded in raw IMU data. LLaSA outperforms commercial LLMs, including GPT-3.5 and GPT-4o-mini, on benchmark and real-world tasks, demonstrating the effectiveness of domain supervision and model alignment for sensor reasoning. Our code repository and datasets can be found at https://github.com/BASHLab/LLaSA.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.14   Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> Tables/context.tex <==
\begin{table}[h]
\centering
\caption{Context Window Sizes for LLMs Evaluated}
\begin{tabular}{|l|c|}
\hline
\textbf{Model}            & \textbf{Context Window} \\
\hline
LLaSA                     & 2048                    \\
GPT-3.5-Turbo             & 16,385                  \\
Vicuna-7/13b-1.5-16K        & 16,384                  \\
GPT-4o-mini               & 128,000                 \\
\hline
\end{tabular}
\label{table:context_window_sizes}
\end{table}

==> Tables/opensqa_prompt.tex <==
\begin{table*}[]
\caption{Prompt design to generate OpenSQA. GPT-4o-mini is prompted with specific instructions and necessary input to generate high-quality five question-answers pair for LLMs.}
\label{tab: opensqa_prompt}
\begin{footnotesize}
\resizebox{\linewidth}{!}{
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{CBCEFB}\textbf{Instruction for Generating OpenSQA}}           \\ \hline
\multicolumn{2} {|p{\textwidth}|}{Please consider yourself an expert on gyroscope and accelerometer sensor information for IMU datasets. You are given the IMU sensor readings of human activity. The user also provides a brief summary of the event followed by 'Summary:' They also give you gyroscopic and accelerometer sensor data followed by 'Gyroscope:' and 'Accelerometer:' respectively. Characteristic IMU features of the event is written after 'Features:' Finally, there's a temporal narration of the events after 'Narration:' Please generate five detailed question-answer pairs that require step-by-step logical deductive thinking and knowledgeable analysis of the sensor data. Please make the questions complex but logical so that they require information that can be derived based on the vast knowledge of sensor data and  IMU activities. The questions and answers need to acknowledge the context given by the user. Please write them in the following list format: 1. Q: Question  A: Answer}
\\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{CBCEFB} \textbf{Prompt Input Structure}}   & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB} \textbf{Output Structure}} \\
\hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}p{0.5\linewidth}@{}}
1. Activity class label\\ 2. Gyroscope sensor data \\ 3. Accelerometer sensor data \\ 4. Sensor Location\\ 5. Characteristic IMU features (SensorCaps) \\ 6. Temporal narration of the activity (SensorCaps)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                    & Five pairs of questions and answers.                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\end{tabular}}
\end{footnotesize}
\end{table*}

==> Tables/prompt_design_close.tex <==
\begin{table*}[]
\caption{Prompt design for zero-shot IMU sensor data classification with LLMs. Classification classes are from the SHL dataset, whereas Other datasets have additional classes. We provide raw sensor data as input GPT models and Vicuna model, and IMU embedding as input LLaSA}
\label{tab:classification_prompt}
\begin{footnotesize}
\resizebox{\linewidth}{!}{
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{CBCEFB}\textbf{Instruction}}           \\ \hline
\multicolumn{2} {|p{\textwidth}|}{\begin{tabular}[c]{@{}l@{}}
The given IMU sensor data can be associated with one of the following classes: 
"standing", "sitting", "walking", "run", "bike", "Unclear". \\
Write only the name of the identified class in the format 
\texttt{"The identified class is: <class\_name>"}.
\end{tabular}}
\\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{CBCEFB} \textbf{Input}}   & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB} \textbf{Output}} \\
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}p{0.5\textwidth}@{}}
LLaSA: IMU embeddings (194 tokens) \\
Other LLMs: Subsampled raw sensor data (~2175 tokens)   \end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                    & The identified class is: \texttt{<class\_name>}                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\end{tabular}}
\end{footnotesize}
\end{table*}

==> Tables/prompt_design_open.tex <==
\begin{table*}[]
\caption{Prompt design for sensor-aware QA evaluation. GPT-4o is prompted with specific instruction to evaluate the quality of the answer generated by LLaSA, GPT-3.5-Turbo and GPT-4o-mini using a quality score and brief summary of the assessement.}
\label{table:openended_assessment_prompt}
\begin{footnotesize}
\resizebox{\linewidth}{!}{
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{CBCEFB}\textbf{Instruction for Assessing Sensor-aware Multimodal LLMs}}           \\ \hline
\multicolumn{2} {|p{\textwidth}|}{\begin{tabular}[c]{@{}p{\textwidth}@{}}
Assume that you are an expert at assessing the quality of predicted answers based on questions related to IMU data and given information. Please use the ’Standard Answer,’ ’Activity Label,’ and ’Sensor Location’ to assess the ’Predicted Answer’ based on the correctness, completeness, consistency, and helpfulness of the predicted answer. Every question is given accelerometer and gyroscope data. So, do not only look at the general answer; check if the answer provided any insights from the data. Provide a single overall score for each answer on a scale of 0 to 100 using the following format: \\
\texttt{Quality score: } \\
Then, give a brief summary of the assessment in 1-2 sentences, followed by "Assessment:". Be specific in evaluating the accuracy, detail, and relevance of the predicted answer in relation to the expected standard. 
\end{tabular}}
\\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{CBCEFB} \textbf{Prompt Input Structure}}   & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB} \textbf{Output Structure}} \\
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}p{0.5\textwidth}@{}}
1. Standard Answer \\
2. Activity Label \\
3. Sensor Location \\
4. Predicted Answer \\
\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}p{0.5\textwidth}@{}}
1. Quality score (0-100) \\
2. Assessment Summary: brief evaluation of answers' 
quality based on correctness, completeness, 
consistency, \\ and helpfulness
\end{tabular}                                                                                                                                                                                                                                                                                                               \\ \hline
\end{tabular}}
\end{footnotesize}
\end{table*}


==> Tables/tune_sqa.tex <==
\begin{table*}[]
\caption{Prompt Design for Tune-OpenSQA Dataset Generation. GPT-4o is prompted to generate QA pairs that focus on different reasoning dimensions for hyperparameter tuning in LLaSA.}
\label{table:sensor_baseline_prompts}
\begin{footnotesize}
\resizebox{\linewidth}{!}{
\begin{tabular}{|p{0.3\textwidth}|p{0.7\textwidth}|}
\hline
\cellcolor[HTML]{CBCEFB} \textbf{Category} & \cellcolor[HTML]{CBCEFB} \textbf{Prompt Instruction} \\
\hline
\textbf{Scientific Reasoning} & "You're an expert on the scientific knowledge behind analyzing IMU sensor data. The IMU sensors are located at {sensor location}. Based on the data and given summary, please generate 5 question-answer pairs that require scientific reasoning. These questions should relate to principles of motion, biomechanics, or physics that explain the correlation between human activity and sensor readings." \\
\hline
\textbf{Narrative Interpretation} & "You're an expert at narrating IMU sensor data for human activities. The IMU sensors are located at {sensor location}. Based on the data and given summary, please generate 5 question-answer pairs that describe what is happening. The questions should require expert interpretation, emphasizing the correlation between movement patterns and real-world activities." \\
\hline
\textbf{Reliability Assessment} & "You're an expert at analyzing the reliability of collected IMU data. The IMU sensors are located at {sensor location}. Based on the data and given summary, please generate 5 question-answer pairs that critically examine whether the given data is trustworthy in the context of the labeled human activity. The questions should assess noise, consistency, and potential anomalies in sensor readings." \\
\hline
\cellcolor[HTML]{E8E8E8} \textbf{Input Structure} & \cellcolor[HTML]{E8E8E8} \textbf{Output Structure} \\
\hline
\cellcolor[HTML]{F5F5F5} 1. Activity Label & \multirow{4}{*}{Five question-answer pairs aligned with the reasoning category.} \\
\cellcolor[HTML]{F5F5F5} 2. Gyroscope Data & \\ 
\cellcolor[HTML]{F5F5F5} 3. Accelerometer Data & \\ 
\cellcolor[HTML]{F5F5F5} 4. Sensor Location & \\
\hline
\end{tabular}}
\end{footnotesize}
\end{table*}

==> _GenAI4HS_25__Mew_LLaSa/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> _GenAI4HS_25__Mew_LLaSa/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.14   Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> _GenAI4HS_25__Mew_LLaSa/Tables/context.tex <==
\begin{table}[h]
\centering
\caption{Context Window Sizes for LLMs Evaluated}
\begin{tabular}{|l|c|}
\hline
\textbf{Model}            & \textbf{Context Window} \\
\hline
LLaSA                     & 2048                    \\
GPT-3.5-Turbo             & 16,385                  \\
Vicuna-7/13b-1.5-16K        & 16,384                  \\
GPT-4o-mini               & 128,000                 \\
\hline
\end{tabular}
\label{table:context_window_sizes}
\end{table}

==> _GenAI4HS_25__Mew_LLaSa/Tables/dataset_table.tex <==
\begin{table}[t]
\caption{Datasets are used to generate SensorCap and OpenSQA. Bolded activities are unseen during training \& tuning. Total 188,429 activities from 95 users.}
\label{tab:opensqa_sources}
\begin{footnotesize}
\begin{tabular}{|l|p{4cm}|c|c|}
\hline
\textbf{Dataset} & \textbf{Classes} & \textbf{Train} & \textbf{Test} \\
\hline
HHAR \cite{stisen2015smart}& bike, sit, stand, walk, ascend stairs, descend stairs & \tmark & \xmark  \\
\hline
Motion \cite{malekzadeh2019mobile} & sit, stand, ascend stairs, descend~stairs, walk, jog & \tmark & \xmark \\
\hline
Shoaib \cite{shoaib2014fusion}& sit, stand, jog, bike, ascend stairs, descend~stairs, walk & \tmark & \xmark  \\
\hline
UCI \cite{reyes2016transition}& stand, sit, lay, walk, ascend stairs, descend stairs & \tmark & \xmark \\
\hline
PAMAP2 \cite{chowdhery2023palm} & lay, sit, stand, walk, run, cycle, Nordic walk, watch TV, computer work, etc. & \tmark & \tmark  \\
\hline
% SHL \cite{gjoreski2018university} & stand, sit, walk, run, bike & \xmark & \tmark  \\
% \hline This is used for close-ended test. We don't create QA pairs from this.
In-the-Wild& sit, stand, \textbf{pick object}, jump, \textbf{swirl}, \textbf{stretch}, use stair, \textbf{elevator}, walk & \xmark  & \tmark \\
\hline
\end{tabular}
\end{footnotesize}
% \vspace{-1.5em}
\end{table}

==> _GenAI4HS_25__Mew_LLaSa/Tables/opensqa_prompt.tex <==
\begin{table*}[]
\caption{Prompt design to generate OpenSQA. GPT-4o-mini is prompted with specific instructions and necessary input to generate high-quality five question-answers pair for LLMs.}
\label{tab: opensqa_prompt}
\begin{footnotesize}
\resizebox{\linewidth}{!}{
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{CBCEFB}\textbf{Instruction for Generating OpenSQA}}           \\ \hline
\multicolumn{2} {|p{\textwidth}|}{Please consider yourself an expert on gyroscope and accelerometer sensor information for IMU datasets. You are given the IMU sensor readings of human activity. The user also provides a brief summary of the event followed by 'Summary:' They also give you gyroscopic and accelerometer sensor data followed by 'Gyroscope:' and 'Accelerometer:' respectively. Characteristic IMU features of the event is written after 'Features:' Finally, there's a temporal narration of the events after 'Narration:' Please generate five detailed question-answer pairs that require step-by-step logical deductive thinking and knowledgeable analysis of the sensor data. Please make the questions complex but logical so that they require information that can be derived based on the vast knowledge of sensor data and  IMU activities. The questions and answers need to acknowledge the context given by the user. Please write them in the following list format: 1. Q: Question  A: Answer}
\\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{CBCEFB} \textbf{Prompt Input Structure}}   & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB} \textbf{Output Structure}} \\
\hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}p{0.5\linewidth}@{}}
1. Activity class label\\ 2. Gyroscope sensor data \\ 3. Accelerometer sensor data \\ 4. Sensor Location\\ 5. Characteristic IMU features (SensorCaps) \\ 6. Temporal narration of the activity (SensorCaps)\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                    & Five pairs of questions and answers.                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\end{tabular}}
\end{footnotesize}
\end{table*}

==> _GenAI4HS_25__Mew_LLaSa/Tables/prompt_design_close.tex <==
\begin{table*}[]
\caption{Prompt design for zero-shot IMU sensor data classification with LLMs. Classification classes are from the SHL dataset, whereas Other datasets have additional classes. We provide raw sensor data as input GPT models and Vicuna model, and IMU embedding as input LLaSA}
\label{tab:classification_prompt}
\begin{footnotesize}
\resizebox{\linewidth}{!}{
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{CBCEFB}\textbf{Instruction}}           \\ \hline
\multicolumn{2} {|p{\textwidth}|}{\begin{tabular}[c]{@{}l@{}}
The given IMU sensor data can be associated with one of the following classes: 
"standing", "sitting", "walking", "run", "bike", "Unclear". \\
Write only the name of the identified class in the format 
\texttt{"The identified class is: <class\_name>"}.
\end{tabular}}
\\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{CBCEFB} \textbf{Input}}   & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB} \textbf{Output}} \\
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}p{0.5\textwidth}@{}}
LLaSA: IMU embeddings (194 tokens) \\
Other LLMs: Subsampled raw sensor data (~2175 tokens)   \end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                    & The identified class is: \texttt{<class\_name>}                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\end{tabular}}
\end{footnotesize}
\end{table*}

==> _GenAI4HS_25__Mew_LLaSa/Tables/prompt_design_open.tex <==
\begin{table*}[]
\caption{Prompt design for sensor-aware QA evaluation. GPT-4o is prompted with specific instruction to evaluate the quality of the answer generated by LLaSA, GPT-3.5-Turbo and GPT-4o-mini using a quality score and brief summary of the assessement.}
\label{table:openended_assessment_prompt}
\begin{footnotesize}
\resizebox{\linewidth}{!}{
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{CBCEFB}\textbf{Instruction for Assessing Sensor-aware Multimodal LLMs}}           \\ \hline
\multicolumn{2} {|p{\textwidth}|}{\begin{tabular}[c]{@{}p{\textwidth}@{}}
Assume that you are an expert at assessing the quality of predicted answers based on questions related to IMU data and given information. Please use the ’Standard Answer,’ ’Activity Label,’ and ’Sensor Location’ to assess the ’Predicted Answer’ based on the correctness, completeness, consistency, and helpfulness of the predicted answer. Every question is given accelerometer and gyroscope data. So, do not only look at the general answer; check if the answer provided any insights from the data. Provide a single overall score for each answer on a scale of 0 to 100 using the following format: \\
\texttt{Quality score: } \\
Then, give a brief summary of the assessment in 1-2 sentences, followed by "Assessment:". Be specific in evaluating the accuracy, detail, and relevance of the predicted answer in relation to the expected standard. 
\end{tabular}}
\\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{CBCEFB} \textbf{Prompt Input Structure}}   & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB} \textbf{Output Structure}} \\
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}p{0.5\textwidth}@{}}
1. Standard Answer \\
2. Activity Label \\
3. Sensor Location \\
4. Predicted Answer \\
\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}p{0.5\textwidth}@{}}
1. Quality score (0-100) \\
2. Assessment Summary: brief evaluation of answers' 
quality based on correctness, completeness, 
consistency, \\ and helpfulness
\end{tabular}                                                                                                                                                                                                                                                                                                               \\ \hline
\end{tabular}}
\end{footnotesize}
\end{table*}


==> _GenAI4HS_25__Mew_LLaSa/Tables/real_quality.tex <==
\begin{table}[]
\centering
\caption{LLaSA-7B delivers more coherent and reliable responses than Vicuna-13B on in-the-wild data.}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Model} & 
\textbf{Model Size} & 
\textbf{Context Length} & 
\textbf{Narrative} & \textbf{Reliability} & \textbf{Overall} \\ \hline
% 13B & 61.0 & 57.2 & 59.1 \\
Vicuna & 13B & 16K & 72.0 & 78.0 & 75.0 \\ \hline
LLaSA & 7B & 2K & \textbf{78.2} & \textbf{81.7} & \textbf{79.95}\\
\hline
\end{tabular}%
}
\label{tab:realword_results}
\end{table}


==> _GenAI4HS_25__Mew_LLaSa/Tables/tune_sqa.tex <==
\begin{table*}[]
\caption{Prompt Design for Tune-OpenSQA Dataset Generation. GPT-4o is prompted to generate QA pairs that focus on different reasoning dimensions for hyperparameter tuning in LLaSA.}
\label{table:sensor_baseline_prompts}
\begin{footnotesize}
\resizebox{\linewidth}{!}{
\begin{tabular}{|p{0.3\textwidth}|p{0.7\textwidth}|}
\hline
\cellcolor[HTML]{CBCEFB} \textbf{Category} & \cellcolor[HTML]{CBCEFB} \textbf{Prompt Instruction} \\
\hline
\textbf{Scientific Reasoning} & "You're an expert on the scientific knowledge behind analyzing IMU sensor data. The IMU sensors are located at {sensor location}. Based on the data and given summary, please generate 5 question-answer pairs that require scientific reasoning. These questions should relate to principles of motion, biomechanics, or physics that explain the correlation between human activity and sensor readings." \\
\hline
\textbf{Narrative Interpretation} & "You're an expert at narrating IMU sensor data for human activities. The IMU sensors are located at {sensor location}. Based on the data and given summary, please generate 5 question-answer pairs that describe what is happening. The questions should require expert interpretation, emphasizing the correlation between movement patterns and real-world activities." \\
\hline
\textbf{Reliability Assessment} & "You're an expert at analyzing the reliability of collected IMU data. The IMU sensors are located at {sensor location}. Based on the data and given summary, please generate 5 question-answer pairs that critically examine whether the given data is trustworthy in the context of the labeled human activity. The questions should assess noise, consistency, and potential anomalies in sensor readings." \\
\hline
\cellcolor[HTML]{E8E8E8} \textbf{Input Structure} & \cellcolor[HTML]{E8E8E8} \textbf{Output Structure} \\
\hline
\cellcolor[HTML]{F5F5F5} 1. Activity Label & \multirow{4}{*}{Five question-answer pairs aligned with the reasoning category.} \\
\cellcolor[HTML]{F5F5F5} 2. Gyroscope Data & \\ 
\cellcolor[HTML]{F5F5F5} 3. Accelerometer Data & \\ 
\cellcolor[HTML]{F5F5F5} 4. Sensor Location & \\
\hline
\end{tabular}}
\end{footnotesize}
\end{table*}

==> _GenAI4HS_25__Mew_LLaSa/tex/00_abstract.tex <==
\begin{abstract}
Wearable systems can recognize activities from IMU data but often fail to explain their underlying causes or contextual significance. To address this limitation, we introduce two large-scale resources: \textbf{SensorCap}, comprising 35,960 IMU--caption pairs, and \textbf{OpenSQA}, with 199,701 question--answer pairs designed for causal and explanatory reasoning. OpenSQA includes a curated tuning split (Tune-OpenSQA) optimized for scientific accuracy, narrative clarity, and diagnostic insight. Leveraging these datasets, we develop \textbf{LLaSA} (Large Language and Sensor Assistant), a family of compact sensor-aware language models (7B and 13B) that generate interpretable, context-rich responses to open-ended questions grounded in raw IMU data. LLaSA outperforms commercial LLMs, including GPT-3.5 and GPT-4o-mini, on benchmark and real-world tasks, demonstrating the effectiveness of domain supervision and model alignment for sensor reasoning.
\end{abstract}

\begin{CCSXML}{
<ccs2012>
  <concept>
    <concept_id>10003151.10003227.10003344</concept_id>
    <concept_desc>Human-centered computing~Ubiquitous and mobile computing systems and tools</concept_desc>
    <concept_significance>500</concept_significance>
  </concept>
  <concept>
    <concept_id>10010147.10010257.10010293</concept_id>
    <concept_desc>Computing methodologies~Multimodal and cross‑modal learning</concept_desc>
    <concept_significance>300</concept_significance>
  </concept>
  <concept>
    <concept_id>10010147.10010371.10010382</concept_id>
    <concept_desc>Computing methodologies~Machine learning</concept_desc>
    <concept_significance>300</concept_significance>
  </concept>
  <concept>
    <concept_id>10010147.10010178.10010224</concept_id>
    <concept_desc>Computing methodologies~Question answering</concept_desc>
    <concept_significance>200</concept_significance>
  </concept>
</ccs2012}
\end{CCSXML}

\ccsdesc[500]{Human‑centered computing~Ubiquitous and mobile computing systems and tools}
\ccsdesc[300]{Computing methodologies~Multimodal and cross‑modal learning}
\ccsdesc[300]{Computing methodologies~Machine learning}
\ccsdesc[200]{Computing methodologies~Question answering}


\keywords{Multi-Modal Large Language Model; Sensor to Query Alignment; Contextual Question-Answering; Sensor-Language Model; Human Activity Reasoning; Hyper-parameter Tuning; IMU}

==> _GenAI4HS_25__Mew_LLaSa/tex/01_introduction.tex <==
\section{Introduction}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/BIG_PIC.pdf}
    \vspace{-2em}
    \caption{A \textbf{real example} comparing GPT-3.5 and LLaSA on an open-ended walking-pattern query. GPT-3.5 responds generically, while LLaSA grounds its explanation in IMU data—referencing upward acceleration and gyroscope stability to infer balanced movement.}
    \label{fig:intro}
\end{figure}

Imagine asking: \textit{“Did I show signs of abnormal gait while climbing stairs? If so, why?”} A meaningful response grounded in motion data could provide real-time insights without technical expertise. Despite over 19 billion IoT devices~\cite{19billion}, 73\% of wearable IMU data remains underused due to its complexity~\cite{newelectronics}. Enabling access to this underutilized sensor data can enhance decision-making across health, fitness, and rehabilitation domains.

While large language models (LLMs) have advanced multimodal understanding in vision and video~\cite{wang2023chatvideo, bai2023qwen}, sensor-based question answering (SQA) remains underexplored. IMU signals are dense, noisy, and lack inherent semantic structure, making alignment with language challenging. Prior models~\cite{chen2021deep, li2024sensorllm} focus on activity classification and label prediction, limiting their ability to explain behavior or reason over time.

We address this gap by introducing two large-scale datasets for open-ended reasoning over IMU data. \textbf{SensorCap} provides 35,960 IMU–caption pairs describing motion, while \textbf{OpenSQA} includes 199,701 question–answer pairs focused on causal and explanatory reasoning. A curated tuning fold of 19,440 examples promotes scientific accuracy, coherence, and diagnostic relevance.

Using these resources, we train LLaSA‑7B and LLaSA‑13B, multimodal LLMs for open-ended, context-aware  QA grounded in IMU data. LLaSA employs a sensor-aware encoder and projection module to compress high-frequency signals into a shared representation that fits within a 2048-token limit.

Figure~\ref{fig:intro} shows LLaSA’s advantage: Unlike GPT-3.5, LLaSA grounds its response in specific IMU signals, referencing upward acceleration and gyroscopic stability to explain a controlled stair ascent, demonstrating causal, sensor-grounded reasoning.

\noindent\textbf{Our key contributions are:}
\begin{itemize}
\item \textbf{Datasets:} We release \textit{SensorCap} and \textit{OpenSQA}, establishing a benchmark for sensor–language reasoning. The tuning fold supports optimization for explanation quality.
\item \textbf{Method:} We propose a GPT-based tuning strategy that promotes scientific accuracy, narrative coherence, and response reliability, without relying solely on classification labels.
\item \textbf{Model:} We introduce \textit{LLaSA}, the first open-source LLM designed for open-ended reasoning over raw IMU data, capable of zero-shot classification and explanatory QA in real-world scenarios.
\end{itemize}

LLaSA is evaluated against GPT‑3.5, Vicuna‑13B, and GPT‑4o‑mini on scientific depth, narrative quality, and contextual grounding. It outperforms GPT‑3.5 and Vicuna‑13B and surpasses GPT‑4o‑mini in sensor-aware QA. Human evaluations (n=22) show strong preference for LLaSA. Real-world trials with 10 users demonstrate generalization to unseen activities and zero-shot classification. Ablations reveal that lower LoRA ranks improve alignment, and GPT-based scoring outperforms loss-based tuning for quality estimation.

==> _GenAI4HS_25__Mew_LLaSa/tex/03_llasa.tex <==
\section{Large Language and Sensor Assistant}
% \bnote{ADD a small intro paragraph here}
Large Language and Sensor Assistant (LLaSA), available in 7B and 13B variants, processes raw IMU data and user queries to generate grounded responses for versatile wearable sensing applications.

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{figures/Overview.pdf}\
\caption{\textbf{LLaSA Overview:} Raw IMU data is encoded by $f_{\theta}$, projected into a shared space $\mathcal{H}_s$, and fused with query embeddings $\mathcal{H}_q$ before being processed by $f_{\Phi}$ to generate a response $\mathcal{X}_a$.}
\label{fig:architecture}
\end{figure}

\subsection{LLaSA Architecture}
Figure~\ref{fig:architecture} illustrates the LLaSA architecture, which includes a sensor encoder for feature extraction, a query encoder, a projection module for multimodal alignment, and a language model conditioned on both inputs.

\noindent\textbf{Sensor Encoder ${f_{\theta}}$.}
Given IMU signals $x(t) \in \mathbb{R}^{C \times T}$, the frozen encoder $f_{\theta}$ produces: $\mathcal{Z}_s = f_{\theta}(x(t)) \in \mathbb{R}^{\bar{c} \times \bar{k}}$. 
We adopt LIMU-BERT~\cite{xu2021limu}, which uses self-attention to encode temporal and channel-wise patterns in $\mathcal{Z}_s$.

\noindent\textbf{Query Encoder $f_t(\cdot)$.}
User queries $Q$ are tokenized using SentencePiece~\cite{kudo1808sentencepiece} (LLaMA-compatible), producing embeddings $\mathcal{H}_q \in \mathbb{R}^{\bar{c} \times k}$.

\noindent\textbf{Projection and Alignment Layer.}
Following previous works \cite{liu2023llava}, you leverage $2$ layers of fully connected layers, along side \textit{GELU}-activation to project the encoded sensor vector $\mathcal{Z}_s$ to sensor embedding $\mathcal{H}_s = \sigma(\mathcal{W}_p \mathcal{Z}_s)$, where $ \mathcal{W}_p \in \mathbb{R}^{\bar{k} \times k}$ is the learnable parameters of projection and alignment layer.

% To align modalities, we apply a GELU-activated projection:
% \[
% \mathcal{H}_s = \sigma(\mathcal{W}_p \mathcal{Z}_s), \quad \mathcal{W}_p \in \mathbb{R}^{\bar{k} \times k}.
% \]
Then we concatenate sensor and text embeddings to form the fused input $\mathcal{H}_{\text{input}} = [\mathcal{H}_s; \mathcal{H}_q]$
This projection acts as a sensor-aware tokenizer, enabling cross-modal consistency.

\noindent\textbf{Language Model $f_{\Phi}$.} The LLM generates output $\mathcal{X}_a$ through autoregressive decoding by modeling the conditional probability as $P(\mathcal{X}_a | \mathcal{H}_{\text{input}}) = \prod_{t=1}^{T} P(x_{a,t} | \mathcal{H}_{\text{input}}, x_{a,<t}; \phi)$ where $\phi$ represents the model parameters. Conditioning on the sensor history $\mathcal{H}_s$ allows for grounded, context-aware reasoning over IMU inputs.


==> _GenAI4HS_25__Mew_LLaSa/tex/04_dataset_generation.tex <==
\section{Sensor-Language Datasets}\label{sec:dataset}

Understanding motion from IMU data requires more than activity classification. It involves contextual reasoning, narrative interpretation, and causal explanation. Existing datasets are largely limited to discrete labels, offering little support for natural language interaction or open-ended tasks. We introduce two large-scale datasets, \textbf{SensorCap} and \textbf{OpenSQA}, that enable training and evaluation of language models for sensor-based reasoning. All datasets are publicly available.\footnote{\href{https://github.com/BASHLab/LLaSA}{https://github.com/BASHLab/LLaSA}}

% \input{Tables/opensqa_prompt}
\subsection{Source HAR Datasets}

Both SensorCap and OpenSQA are derived from six publicly available human activity recognition (HAR) datasets and one dataset we collected in the wild, as summarized in Table~\ref{tab:opensqa_sources}. The in-the-wild dataset introduces natural noise and variability, allowing us to assess model robustness, reliability, and real-world applicability in the test set. We recruited 10 adults through campus bulletin boards and social media. Each participant used their personal smartphone to record sensor data with the Sensor Logger app~\cite{tszheichoiSensorLogger} while performing \textit{nine} predefined activities, each lasting two minutes (activity list shown in Table~\ref{tab:opensqa_sources}). Recordings took place in diverse environments—approximately 70\% on campus and 30\% at home. Devices varied across iPhone, Samsung, and Google Pixel models, capturing a wide range of hardware and sensor characteristics.


\subsection{SensorCap: Sensor Data Captioning}

SensorCap consists of 35,960 IMU–caption pairs. Each sample includes raw accelerometer and gyroscope signals, sensor location, derived features (e.g., FFT, min, max, median, and variance) and the activity label. The numerical data are downsampled to 10 Hz and truncated to 6 digits after the decimal point.  For each instance, we generate two types of natural language outputs: (1) \textit{a summary caption of at most 25 words describing dominant motion patterns}, and (2) \textit{a step-by-step narration of up to 500 tokens explaining sensor dynamics over time}.

To generate SensorCap, we prompted GPT-4o-mini with characteristic IMU features (e.g., FFT, maxima, variance), raw gyroscope and accelerometer data, and a brief activity summary. To input sensor data into GPT-4o-mini, we converted time-series IMU readings (accelerometer and gyroscope) into structured JSON-like arrays with up to 100 time steps. Additional features such as FFT, statistical summaries (mean, max, min, variance), and sensor locations were appended as human-readable feature descriptors. This structured input was paired with an activity label and passed as the context to GPT-4o-mini. The model generated multi-paragraph explanations grounded in both temporal signal patterns and derived statistical features. For example, the input:

\texttt{Summary: biking; Gyroscope: [[...]]; Accelerometer: [[...]]; Features: FFT, max, min, median, moving avg, variance}

produces a multi-paragraph response narrating rotational and linear acceleration patterns consistent with biking. The model identified z-axis gravitational force, lateral motion for turns, and gyroscopic peaks suggesting leaning behavior and terrain adaptation. The narration also referenced oscillations, balance corrections, and exertion cues tied to real-world biking dynamics.

These structured narrations form the input for our prompt suite, which supports OpenSQA question-answer generation. Each prompt conditions GPT-4o-mini with SensorCap-derived descriptions and guides it to produce QA pairs grounded in sensor reasoning across dimensions such as biomechanics, reliability, and contextual interpretation.


\input{Tables/dataset_table}

\subsection{OpenSQA: Sensor-Aware QA Dataset}

OpenSQA extends SensorCap to support open-ended question answering grounded in IMU data. It contains 199,701 question–answer pairs, each generated using gyroscope and accelerometer signals, activity labels, sensor locations, and SensorCap-provided motion features and narrations. Each QA pair is a natural language response to a user-style question grounded in this multimodal sensor context. For each instance, we prompt GPT-4o-mini to generate five QA pairs spanning factual (e.g., \textit{“What activity is being performed?”}), descriptive (e.g., \textit{“What trends are visible?”}), causal (e.g., \textit{“Why is this motion occurring?”}), diagnostic (e.g., \textit{“Is this motion stable or noisy?”}), and inferential (e.g., \textit{“What might happen next?”}) reasoning. A subset of generations is refined with human feedback to improve clarity and contextual alignment. 

To support structured evaluation beyond label prediction, we partition OpenSQA into two folds: A \textbf{training fold} includes \textbf{179,727} QA pairs constructed from five datasets: HHAR, MotionSense, Shoaib, UCI HAR, and the training portion of PAMAP2~\cite{chowdhery2023palm}, and a \textbf{tuning fold}, \textbf{Tune-OpenSQA}, contains 19,440 QA pairs generated from a held-out PAMAP2 subset with GPT-4o. It serves as a benchmark for evaluating sensor-aware reasoning across scientific consistency, narrative clarity, and signal reliability.

For further real-world assessment, we include an in-the-wild dataset of \textbf{534 QA pairs}. This subset evaluates model generalization under diverse environmental conditions and device variation.



\subsection{Data Quality Assessment}

We assess dataset quality using three LLMs as automatic judges: Deepseek-V3 (accessed via API), LLaMA-3.1-8B, and Gemma-12B (run locally). Each model scores question–answer pairs on a 1-5 scale based on alignment with IMU data, activity label, and narration. Deepseek-V3 rates 87\% of samples above 4.5 and 96\% above 4.0. Gemma-12B scores 73\% above 4.5 and 93\% above 4.0. LLaMA-3.1-8B gives 97\% above 4.5 and 100\% above 4.0. The consistency across models confirms the high quality of the generated data and its suitability for sensor-grounded reasoning tasks.

==> _GenAI4HS_25__Mew_LLaSa/tex/05_result.tex <==
\section{Evaluation for Open-Ended Reasoning Question Answering}

We evaluate LLaSA’s ability to generate interpretable, context-rich answers from raw IMU data. Unlike standard classification, this task involves open-ended questions that require causal reasoning and contextual understanding. Our evaluation framework includes three components: (1) a structured LLM-based evaluation metric (Section~\ref{sec:hyperparam}), (2) human satisfaction ratings, and (3) generalization to in-the-wild settings with unseen activities that test LLaSA’s ability to reason about novel motion patterns. We also assess LLaSA’s performance on zero-shot human activity classification. While LLaSA uses normalized 20 Hz samples to generate sensor tokens, others receive them as texts downsampled to 10 Hz and truncated up to 6 digits after the decimal point to minimize the number of tokens.

\begin{table}[]
\centering
\caption{LLaSA leads in science score and overall quality, outperforming stronger-context LLMs.}
\label{table:quality_scores}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Context Len.} & \textbf{Science} & \textbf{Narration} & \textbf{Reliability} & \textbf{Overall} \\ \hline
LLaSA & 2k & \textbf{75.0} & 71.0 & 70.5 & 72.17 \\ \hline
GPT-3.5-Turbo & 16k & 64.5 & 65.0 & 60.0 & 63.17 \\ \hline
GPT-4o-mini & 128k & 72.0 & \textbf{77.0} & \textbf{78.0} & 75.67 \\ \hline
Vicuna-13b & 16k & 63.4 & 67.0 & 65.4 & 65.27 \\ \hline
\end{tabular}
}]
\end{table}

\subsection{Comparison with General LLMs}

We compare LLaSA‑13B to GPT‑3.5, GPT‑4o‑mini, and Vicuna‑13B using a structured evaluation of scientific reasoning, narrative clarity, and reliability (Table~\ref{table:quality_scores}). All models are scored on 30 QA pairs from the OpenSQA tuning fold (PAMAP2 data).

LLaSA outperforms GPT‑3.5 and Vicuna‑13B across all metrics, producing more sensor-aware and causally grounded answers. It leads in scientific reasoning, highlighting the value of domain-specific tuning. GPT‑4o‑mini performs well but lacks depth in physics reasoning, showing general models benefit from domain adaptation.

Despite a 2K context limit, LLaSA matches or exceeds models with up to 64$\times$ larger context windows. Its strong performance—without architectural changes—demonstrates that careful tuning can enable compact models to reason accurately over sensor data.

\begin{figure}[]
\centering
\includegraphics[width=0.5\textwidth]{figures/llasa_survey.pdf}
\caption{LLaSA yields more consistent high human satisfaction scores than baselines.}
\label{fig:survey_result}
\end{figure}

\begin{figure*}[!htb]
\centering
\includegraphics[width=\textwidth]{figures/qa-vaccum.pdf}
\caption{Example showing LLaSA provides enriched, contextual answers (\textbf{highlighted in red}) based on IMU input.}
\label{fig:qa_example}
\end{figure*}

\subsection{Human Evaluation of QA Quality}

We conducted a user study with 21 participants to evaluate the perceived quality of sensor-based answers. Each participant reviewed 10 QA examples covering scientific reasoning, narrative clarity, and reliability. Questions were paired with anonymized outputs from LLaSA-13B, GPT-3.5, GPT-4o-mini, and Vicuna-13B. Visual plots and brief IMU descriptions aided interpretation.

Participants ranked answers from 1 (worst) to 4 (best) based on clarity, relevance, and grounding. LLaSA scored highest in 40\% of cases, matching GPT-4o-mini, but with fewer low scores, showing greater consistency. Figure~\ref{fig:survey_result} highlights LLaSA’s precision in interpreting subtle sensor cues.

Figure~\ref{fig:qa_example} shows an example: while Vicuna-13B offers a generic explanation, LLaSA cites specific signal fluctuations—e.g., z-axis acceleration and gyroscope variance—to infer obstacles and strenuous activity during vacuum cleaning.

Participants noted that LLaSA improved their understanding by linking low-level signals to high-level explanations. Even non-experts found its answers more informative and accessible, reinforcing the value of domain-specific tuning for real-world use.

\input{Tables/real_quality}

\subsection{Generalization to In-the-Wild Data}
We evaluate LLaSA-7B on an OpenSQA test fold that includes only in-the-wild samples collected using smartphones in real-world environments. This evaluation assesses narrative quality and reliability under noise and device variations.

We compare LLaSA-7B with Vicuna-13B-1.5-16K, a significantly larger general-purpose model. To ensure fairness, GPT-4o scores the outputs using prompts designed to account for variability in real-world sensor signals. As shown in Table~\ref{tab:realword_results}, LLaSA delivers more coherent and reliable answers across a wide range of activities, despite its smaller model size and limited context window. These results highlight LLaSA’s ability to generalize beyond curated datasets and maintain performance in practical deployment scenarios.

\input{tex/result_table}

\subsection{Zero-Shot Activity Classification}

We evaluate LLaSA’s ability to perform zero-shot activity recognition, where the model classifies IMU signals without task-specific fine-tuning by selecting the most plausible activity label.

We use five datasets: HHAR, Motion, Shoaib, UCI, and SHL~\cite{gjoreski2018university}. Each sample includes derived IMU features and candidate activity labels (Table~\ref{tab:opensqa_sources}). The model is prompted to choose the correct label; if none is returned, the output is marked “Unclear.” Performance is measured using precision, recall, and F1-score.

Compared to Vicuna-7B, GPT-3.5, GPT-4o-mini, and a fine-tuned GPT-3.5 (GPT-3.5-T-F), LLaSA achieves 2.6–12$\times$ higher F1 across all datasets (Table~\ref{tab:closeendedresults}). It generalizes well even to SHL, unseen during training. Despite a 2K token limit, LLaSA outperforms models with up to 128K context length, demonstrating strong efficiency and domain grounding.

\input{tex/table_finetune}

\section{Tuning Strategy Evaluation and Insights}
We study how LoRA rank, model size, and dataset scale influence performance. LLaSA is fine-tuned on 30 QA examples spanning diverse reasoning types, varying LoRA rank, learning rate, and model size (Table~\ref{table:hyperparams}). Rank 8 consistently performs best across science, narration, and reliability, supporting prior findings that low-rank adaptation improves alignment and reduces overfitting on noisy IMU data. The 13B model outperforms 7B across all metrics, though both benefit from tuning. Expanding to the full PAMAP2 QA dataset (179k examples) offers marginal improvement, suggesting saturation beyond a certain scale.

Notably, the lowest-loss model (1.474) performs worse than the best one (1.526), confirming that training loss is an unreliable proxy for QA quality. Our structured quality scores better reflect interpretability, grounding, and reasoning, and are more suitable for tuning sensor-aware language models.


==> _GenAI4HS_25__Mew_LLaSa/tex/06_related.tex <==
\section{Related Work}

Recent research has explored leveraging large language models for sensor-grounded reasoning tasks. Penetrative AI~\cite{xu2024penetrative} demonstrated that models like ChatGPT can interpret textualized IoT sensor data to perform perception and activity inference tasks in physical domains. RAVEN~\cite{biswas2025raven} introduces a cross-modal gating mechanism over audio, video, and sensor streams, showing significant improvement in multimodal QA accuracy by weighting relevant modalities.

In the sensor-Language alignment space, LLMSense~\cite{ouyang2024llmsense} incorporates long-term spatiotemporal sensor traces through selective history inclusion and summarization before reasoning on the cloud, achieving over 80\% accuracy in tasks like dementia diagnosis and occupancy tracking. SensorLLM~\cite{zhang2025sensorlm} aligns sensor channel data with LLMs using special tokens and trend-descriptive text, enabling robust activity recognition without manual annotations.

Other systems—such as IMUGPT2.0~\cite{leng2024imugpt}, Sensor2Text~\cite{chen2024sensor2text}, and MentalLLM~\cite{xu2024mental}—focus on generating summaries or labels from sensor data, but lack the open‑ended reasoning and QA functionality that LLaSA supports.

A unique approach called By My Eyes~\cite{yoon-etal-2024-eyes} converts IMU and ECG signals to visual prompts for multimodal LLMs, whereas LLaSA directly models raw sequences without modality conversion

In healthcare, models like Health‑LLM~\cite{kim2024health}, MedTSLLM~\cite{chan2024medtsllm}, PH‑LLM~\cite{cosentino2024towards}, and PHIA~\cite{merrill2024transforming} fine-tune LLMs on wearable sensor data for structured clinical prediction. Surveys such as Zhang et al.~\cite{zhang2024large} review LLM applications to time series, but highlight that most existing methods focus on task-level prediction or forecasting rather than temporally grounded explanations or QA.



==> _GenAI4HS_25__Mew_LLaSa/tex/07_conclusion.tex <==
\section{Limitations}
One limitation of our approach is the reliance on a single LLM, GPT-4o-mini, for both SensorCap generation and OpenSQA QA synthesis. While GPT-4o offers high-quality reasoning, its performance and tokenization biases inherently influence the quality of the datasets. While inter-rater reliability between GPT and Deepseek was good (0.92), evaluation using GPT-based automatic metrics also inherits this dependency, which may affect reproducibility as models evolve over time.
Another limitation is the scale of human evaluation and benchmark QA comparison. The current evaluation spans 30 QA pairs for benchmarking and 10 examples per human rater, which may limit statistical robustness. Expanding this in future work will help validate the generalization of LLaSA.
We also observe that LLaSA occasionally fails in ambiguous or under-informative input scenarios, such as stationary readings misclassified as “standing” vs. “sitting.” It may also hallucinate motion patterns when the signal lacks clear transitions, or overfit to statistically common movement descriptors even when context differs. Addressing such failure modes is an avenue for future improvement, especially with fine-grained signal conditioning or counterfactual prompts.
Finally, the current model sizes (7B and 13B with 16-bit precision) are unsuitable for real-time inference on mobile or edge devices. Supporting deployment on smartphones or wearables would require model compression strategies such as quantization, distillation, or architecture pruning. Exploring efficient sensor-language reasoning under these constraints is an important direction for future work, particularly for privacy-preserving, on-device applications.


\section{Conclusion}
We present SensorCaps and OpenSQA, two new resources that enable sensor-grounded question answering with open-ended, causal reasoning over IMU data. Built on these datasets, LLaSA shows how lightweight adaptation and structured evaluation can produce interpretable, context-rich answers from raw sensor signals. LLaSA outperforms general-purpose LLMs up to 64$\times$ larger while remaining efficient and real-time capable. These results highlight the value of domain-specific supervision for aligning language models with low-level sensor data. Future work will extend this foundation to support multimodal fusion, interactive dialogue, and longer contexts for deployment in health, HCI, and wearable systems.

\section*{Acknowledgment}
This research was supported by funding from the NSF CNS-2347692. We gratefully acknowledge their support in enabling this work.


==> _GenAI4HS_25__Mew_LLaSa/tex/09_realworld.tex <==
\input{tex/result_table}
\subsection{Generalization to Real-World Data}

\parlabel{Data Collection}
To test real-world applicability, we collect a new dataset from 10 adult participants using personal smartphones and the Sensor Logger app~\cite{tszheichoiSensorLogger}. Participants, recruited via campus boards and social media, recorded \textit{nine} predefined activities (Table~\ref{tab:opensqa_sources}) in familiar settings—70\% on campus, 30\% at home. Devices included iPhone, Samsung, and Pixel models, capturing diverse hardware conditions.

Each activity lasted ~2 minutes and was performed in a fixed order while holding the phone. This setup introduces natural variability and noise, particularly relevant to the “Reliability” aspect of QA. The dataset, reflecting a range of real-world scenarios, is available in our repository.

\noindent\textbf{Data Processing.}
We discard the first/last 2 seconds of each recording, then split the remaining data into 6-second segments and downsample from 100Hz to 20Hz for consistency. From ~20 segments per activity per user, we sample a few and generate 3 QA pairs (focused on reliability and narration), resulting in 534 total QA examples grounded in user-collected smartphone IMU data.

\parlabel{Evaluation}
We evaluate LLaSA-7b against Vicuna-13b-1.5-16K on 50 randomly chosen QA pairs per category, using the quality metric from Section~\ref{sensor-qa-eval-scoring}. All QAs are derived from real-world smartphone accelerometer and gyroscope readings. To account for sensor and context variability, we prompt GPT-4o to adjust expectations during scoring. As shown in Table~\ref{tab:realword_results}, LLaSA performs comparably or better than on curated PAMAP2 data—demonstrating its robustness to uncontrolled, noisy input and outperforming larger general-purpose models despite a smaller context window and compressed feature input.


==> _GenAI4HS_25__Mew_LLaSa/tex/Experimental_setup.tex <==
\section{Experimental Setup}
\subsection{Experiments}
We conduct a series of experiments to evaluate LLaSA on both open-ended and close-ended QA, fine-tune model parameters, assess model scalability, and validate performance in real-world scenarios.

\noindent\textbf{Open-Ended QA:} We evaluate the model’s ability to generate contextual responses from raw sensor data. Given sensor inputs corresponding to different human activities, the model is prompted with open-ended questions requiring reasoning about the activity context. The objective is to assess the model’s capacity for understanding, inference, and contextual awareness beyond direct classification. For automated evaluation, we utilize 30 QA pairs distributed evenly among the categories. To simplify human evaluation, we pick a subset of 10 QA pairs that represent the range of GPT-assisted scores our model achieved while also ensuring diversity of human activities, sensor locations, and evaluation categories.

\noindent\textbf{Close-Ended QA: } We perform zero-shot classification on raw sensor data for human activity recognition, where zero-shot means that we do not explicitly train the model for classification. The model is prompted with predefined activity categories and asked to classify the given IMU signals accordingly. This experiment assesses the model’s capability to generalize to unseen data and recognize activities without explicit fine-tuning on labeled datasets.

\noindent\textbf{Hyper-parameter Tuning} To optimize model performance for IMU-related question-answering tasks, we fine-tune key hyperparameters, including learning rate, batch size, and sequence length, using our . The goal is to maximize inference quality and efficiency, ensuring that the model effectively processes and responds to IMU-based queries.

\noindent\textbf{Model Scaling: } We investigate the impact of model size on question-answering performance by evaluating different configurations of the model. This experiment explores how larger model variants influence accuracy, response coherence, and computational efficiency, providing insights into the trade-offs between model complexity and performance.

\noindent\textbf{Real-Word Evaluation: } To assess real-world generalization, we collect a new dataset comprising human activity data from participants of diverse backgrounds, performing activities in varied real-world scenarios while carrying a mobile phone. The collected data is used to benchmark our approach against existing baseline models. Performance is evaluated based on both open-ended responses and classification accuracy, providing a comprehensive comparison of model robustness in realistic conditions.

\subsection{Datsets}
We evaluate LLaSA on our proposed OpenSQA dataset for open-ended tasks (details in section \ref{opensqa-dset}) and close-ended tasks were evaluated on $5$ publicly available human activity recognition datasets.

\noindent\textbf{HHAR ~\cite{stisen2015smart}.} The HHAR dataset includes accelerometer and gyroscope recordings from $9$ users performing $6$ activities: biking, sitting, standing, walking, climbing upstairs, and going downstairs. Data was collected using $6$ smartphone models, worn around the waist with sampling rates ranging from $100$ Hz to $200$ Hz.

\noindent\textbf{MostionSense ~\cite{malekzadeh2019mobile}.} ollected using an iPhone 6s, this dataset contains accelerometer and gyroscope time-series data from 24 participants of diverse gender, age, weight, and height. Participants performed 6 activities (walking, jogging, sitting, standing, going upstairs, and going downstairs) with the phone in their front pocket, recorded at 50 Hz.

\noindent\textbf{Shoaib ~\cite{shoaib2014fusion}.} his dataset captures 7 physical activities (walking, sitting, standing, jogging, biking, walking upstairs, and walking downstairs) from 10 male participants. Each participant carried 5 Samsung Galaxy S II smartphones placed at different body positions (right pocket, left pocket, belt, upper arm, and wrist). Data includes accelerometer, gyroscope, and magnetometer readings, recorded at 50 Hz.

\noindent\textbf{UCI ~\cite{reyes2016transition}.} This dataset includes accelerometer and gyroscope data from 30 volunteers (ages 19–48) performing 6 activities (standing, sitting, lying, walking, walking upstairs, and walking downstairs). Data was collected using a Samsung Galaxy S II worn on the waist, with a constant sampling rate of 50 Hz.

\noindent\textbf{SHL ~\cite{gjoreski2018university}.} A large-scale multi-sensor dataset includes various sensor modalities such as accelerometer, gyroscope, orientation, gravity, and GPS. It captures activities like sitting, walking, and running, both in every day and transportation scenarios, such as traveling by bus or train. 

\subsection{Baselines}
\noindent\textbf{Vicuna-7b-16k ~\cite{}} Vicuna 7B-16K is an open-source large language model (LLM) based on Llama 2, designed for efficient and high-quality text generation. It features 7 billion parameters and supports an extended 16K token context window, enabling it to handle longer conversations and documents effectively.

\noindent\textbf{GPT 3.5-T ~\cite{}} GPT-3.5-T is a variant of OpenAI’s GPT-3.5 model, optimized for efficiency and performance in text generation, reasoning, and conversation tasks.  While specific details about its architecture and parameter count may vary, it is designed to handle complex queries, assist in coding, generate high-quality text, and support multi-turn interactions effectively.

\noindent\textbf{GPT-4o-mini ~\cite{}}


\noindent\textbf{GPT-4o ~\cite{}}

\noindent\textbf{GPT 3.5-T-F ~\cite{}}


\subsection{Evaluation Metrics}
For the close-ended task, we report the \textit{F1-Score}, \textit{Precision}, and \textit{Recall} for all baselines alongside LLaSA. Additionally, we provide the context length used by each baseline, highlighting the model complexity required to achieve a given level of zero-shot classification performance.

For open-ended tasks such as comparisons with baseline LLMs, real-world evaluation, and hyperparameter tuning to find the best model capable of following sensor-aware instructions, we compare different model sizes using three key metrics: \textit{Narrative QA Score}, \textit{Reliability QA Score}, and their mean, \textit{Overall Score}, ensuring a fair comparison. The scoring system follows the framework we present in Section \ref{subsec:quality_score}. Additionally, we include qualitative examples to provide deeper insights and enhance understanding of the model's responses.

==> _GenAI4HS_25__Mew_LLaSa/tex/Table_sensorcap.tex <==
\begin{table*}[]
\caption{Prompt design for SensorCaps generation. We prompt GPT-4o-mini with specific instructions to generate a caption for the sensor data in 20-25 words and generate a step-by-step narration of the activity's sensor reading.}
\label{tab:sensorcap_propmt}
\begin{footnotesize}
\resizebox{\linewidth}{!}{
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{CBCEFB}\textbf{Instruction for Generating SensorCaps}}           \\ \hline
\multicolumn{2} {|p{\textwidth}|}{\begin{tabular}[c]{@{}p{\textwidth}@{}}
Please consider yourself to be an expert on gyroscope and accelerometer sensor information given as metadata of IMU datasets. You are given the IMU sensor readings of human activity. The user also provides a brief summary of the event followed by 'Summary:'. They also give you gyroscopic and accelerometer sensor data followed by 'Gyroscope:' and 'Accelerometer:' respectively. They are written in a Python list of lists format and contain x, y, and z-axis data, respectively. Please pay attention to the values and the signs. Additional information computed for each axis is provided afterward, with the windows for moving averages being 12. You should provide comprehensive detail of at least a couple of characteristic IMU features for that event within 20-25 words, followed by 'Features:.' The IMU features should be concise and descriptive. Separate multiple features with commas. Derive the list of features based on the given sensor data. Then, narrate the temporal event with details that are context-aware based on the sensor data, followed by 'Narration:' in a step-by-step fashion, analyzing it within 500 words or less. Please analyze even the small movements thoroughly in a logical and contextual manner, utilizing a deductive thought process while being aware of the knowledge regarding the meaning of the sensor data. Use descriptive terms that aren't vague. \\

\end{tabular}}
\\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{CBCEFB} \textbf{Prompt Input Structure}}   & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB} \textbf{Output Structure}} \\
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}p{0.5\linewidth}@{}}1. Activity class label \\ 2. Gyroscope sensor data \\ 3. Accelerometer sensor data\\ 4. Sensor location \\ 5. Handcrafted features: moving averages, FFT, min, max, median, variance for each axis\end{tabular}}                                             & \begin{tabular}[c]{@{}l@{}}1. Characteristics IMU features in natural language \\ 2. Narration of the activity's sensor readings\end{tabular}                                                                                                                                                                                                                                                                                                               \\ \hline
\end{tabular}}
\end{footnotesize}
\end{table*}

==> _GenAI4HS_25__Mew_LLaSa/tex/finetuning.tex <==
\subsection{LLaSA Hyperparameter Tuning}
\label{sec:hyperparam}

Integrating sensor data into LLMs presents challenges beyond standard text-based tuning. Sensor-aware models must process noisy, continuous signals, preserve temporal dependencies, and generate responses grounded in physical context. Prior work often relies on classification labels, limiting a model’s ability to generate explanatory outputs.%% Shortened sentence
We propose a tuning strategy that improves interpretability and reliability without modifying model architecture. It combines targeted hyperparameter search with a structured evaluation protocol to support causal reasoning and multimodal alignment.%% Slightly condensed

\noindent\textbf{Hyperparameter Search Strategy.}
We tune five key parameters to balance convergence and expressivity: learning rate ($\eta$), batch size ($B$), weight decay ($\lambda$), LoRA rank ($r$), and dropout rate ($p_{\text{drop}}$). Following prior work~\cite{sellam2020bleurt}, we select configurations using the evaluation metric below to ensure fidelity in sensor-grounded responses.%% Condensed second sentence

\begin{table}[]
\caption{BLEU/ROUGE reward generic overlap. GPT scoring reflects reasoning and relevance in sensor-grounded QA.}
% \vspace{-1em}
\label{table:evaluation_comparison}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}|l|l|l|@{}}
\toprule
Query &
  Generic Response &
  Informed Response \\ \midrule
\begin{tabular}[c]{@{}l@{}}What is the\\ person doing?\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}"The person is moving."\\ \textbf{BLEU/ROUGE:} High \\ \textbf{GPT:} Low\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}"Smooth gait suggests walking."\\ \textbf{BLEU/ROUGE:} Medium \\ \textbf{GPT:} High\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Is the activity\\ classification\\ correct?\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}"Yes, it matches the label."\\ \textbf{BLEU/ROUGE:} High \\ \textbf{GPT:} Low\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}"Patterns match walking signature."\\ \textbf{BLEU/ROUGE:} Medium \\ \textbf{GPT:} High\end{tabular} \\ \bottomrule
\end{tabular}
}
% \vspace{-1.5em}
\end{table}

\noindent\textbf{Structured LLM-Based Evaluation Metric.}
Lexical metrics like BLEU~\cite{papineni2002bleu} and ROUGE~\cite{lin-2004-rouge} often fail to reflect semantic or causal relevance, especially in sensor-grounded QA where phrasing varies~\cite{gao2024llm, desmond2024evalullm}. As shown in Table~\ref{table:evaluation_comparison}, vague answers like \textit{“The person is moving”} can receive high BLEU scores despite lacking depth.

To address this, we score answers using GPT-4o along four axes: \textit{correctness}, alignment with sensor dynamics; \textit{completeness}, coverage of key observations; \textit{consistency}, logical flow; and \textit{helpfulness}, clarity and informativeness. Each is rated on a 0–100 scale, and the average yields a final score:
\begin{equation*}
Q_{\text{final}} = \frac{Q_{\text{correctness}} + Q_{\text{completeness}} + Q_{\text{consistency}} + Q_{\text{helpfulness}}}{4}
\end{equation*}

This scoring captures coherence, context, and reasoning better than lexical overlap. For instance, \textit{“Smooth gait suggests walking”} scores higher than generic responses. We validate the approach with Deepseek-V3, observing strong inter-rater agreement (ICC = 0.92, \textbf{p} = 0.0001), confirming its reliability.

==> _GenAI4HS_25__Mew_LLaSa/tex/implementation.tex <==
\subsection{Implementation Details}

\noindent\textbf{LIMU-BERT Training.} \label{limubert-training}
We pretrain LIMU-BERT on unlabeled sensor data from HHAR~\cite{stisen2015smart}, UCI-HAR~\cite{reyes2016transition}, MotionSense~\cite{malekzadeh2019mobile}, and Shoaib~\cite{shoaib2014fusion}, covering 8 activities with 3-axis accelerometer and gyroscope signals downsampled to 20 Hz. The best checkpoint is selected after ~8 hours of training (up to 1000 epochs) with Adam and early stopping on an RTX 3090 Ti. Additional PAMAP2 activities~\cite{roggen2010collecting} yielded negligible gains, indicating sufficient diversity in the core datasets.

\noindent\textbf{Multimodal Projector Training.}
We train a GELU-activated MLP ($W_P$) on OpenSQA to align LIMU-BERT sensor features with token embeddings. Training uses 16-bit precision, Adam optimizer, learning rate $1\text{e}^{-4}$, and batch size 32 on A100 GPUs. One epoch suffices for convergence.

\noindent\textbf{LLaSA Fine-Tuning.}
We fine-tune Vicuna-7B and 13B with LoRA~\cite{hu2021lora}, using the pretrained projector and LLaVA-style~\cite{liu2023llava} instruction tuning. Sensor embeddings fit within a 2048-token context window. The 7B model is trained on one A100 GPU; 13B uses two.

Fine-tuning runs for one epoch (batch size 16) with LoRA ranks $r \in \{4, 8, 16, 64, 128\}$ and scaling $\alpha = r$~\cite{lee2023platypus}. We sweep learning rates of $1\text{e}^{-4}$, $3\text{e}^{-5}$, $1\text{e}^{-6}$ for LoRA, and $2\text{e}^{-5}$, $1\text{e}^{-4}$, $1\text{e}^{-3}$ for the projector.



==> _GenAI4HS_25__Mew_LLaSa/tex/result_table.tex <==
\begin{table*}[]
\caption{Zero-shot classification performance on human activity recognition. LLaSA outperforms GPT models and Vicuna-7B with 2.6–12× higher F1-scores, despite using 8–64$\times$ smaller context windows.}
\vspace{-1em}
\label{tab:closeendedresults}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{|@{}l|c|ccc|ccc|ccc|ccc|ccc@{}|}
\toprule
\multicolumn{1}{|c|}{\multirow{2}{*}{LMA}}              &\multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}{@{}l@{}}
                   Context \\
                   length
              \end{tabular}}}  &\multicolumn{3}{|c|}{HHAR}                   & \multicolumn{3}{c|}{MotionSense} & \multicolumn{3}{c|}{Shoaib} & \multicolumn{3}{c|}{UCI}   & \multicolumn{3}{c|}{SHL}   \\ \cmidrule(l){3-17}
\multicolumn{1}{|c|}{}                &\multicolumn{1}{c|}{}  & F-1  & Precision & Recall & F-1    & Precision   & Recall   & F-1   & Precision & Recall & F-1  & Precision & Recall & F-1  & Precision & Recall \\ \hline
Vicuna-7b-16K & 16k            & 0.05 & 0.12      & 0.03   & 0.09   & 0.15        & 0.12     & 0.08  & 0.11      & 0.11   & 0.04 & 0.25      & 0.03   & 0.08 & 0.38      & 0.07   \\ \hline
GPT-3.5-T     & 16k            & 0.07 & 0.16      & 0.1    & 0.08   & 0.07        & 0.13     & 0.09  & 0.1       & 0.12   & 0.07 & 0.35      & 0.12   & 0.15 & 0.22      & 0.15   \\ \hline
GPT-4o-mini   & 128k           & 0.16 & 0.24      & 0.18   & 0.12   & 0.25        & 0.15     & 0.1   & 0.19      & 0.13   & 0.15 & 0.17      & 0.13   & 0.25 & 0.36      & 0.23   \\ \hline
GPT-4o        & 128k           & 0.07 & 0.14      & 0.08   & 0.08   & 0.26        & 0.06     & 0.14  & 0.35      & 0.15   & 0.04 & 0.16      & 0.03   & 0.22 & 0.27      & 0.23   \\ \hline
GPT-3.5-T-F   & 16k            & 0.52 & 0.54      & 0.7    & 0.21   & 0.27        & 0.21     & 0.27  & 0.45      & 0.31   & 0.24 & 0.28      & 0.31   & 0.23 & 0.25      & 0.32   \\ \hline
LLaSA         & \textbf{2k}             & \textbf{0.84} & \textbf{0.88}      & \textbf{0.86}   & \textbf{0.83}   & \textbf{0.85}        & \textbf{0.83}     & \textbf{0.81}  & \textbf{0.84}      & \textbf{0.81}   & \textbf{0.72} & \textbf{0.82}      & \textbf{0.75}   & \textbf{0.65} & \textbf{0.76}      & \textbf{0.71} \\ \bottomrule 
\end{tabular}}

\end{table*}

==> _GenAI4HS_25__Mew_LLaSa/tex/table_finetune.tex <==
\begin{table}[]
\centering
\caption{Hyperparameter tuning and model scaling help find the best-performing model through scientific, narrative, and reliability assessment QA Tasks.}
\vspace{-1em}
\label{table:hyperparams}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c||c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Model\\ size\end{tabular} & \begin{tabular}[c]{@{}c@{}}\#QA\end{tabular} & LR                    & \begin{tabular}[c]{@{}c@{}}Projector\\ LR\end{tabular} & \begin{tabular}[c]{@{}c@{}}LORA\\ Rank\end{tabular} & \begin{tabular}[c]{@{}c@{}}Science \\ QA Quality\end{tabular} & \begin{tabular}[c]{@{}c@{}}Narration\\ QA Quality\end{tabular} & \begin{tabular}[c]{@{}c@{}}Reliability\\ QA Quality\end{tabular} & \begin{tabular}[c]{@{}c@{}}Overall\\ Score\end{tabular} \\ \hline
\multirow{22}{*}{7b}                                 & \multirow{12}{*}{131,407}                                 & \multirow{6}{*}{1e-4} & \multirow{3}{*}{1e-4}                                  & 8    & 41.0                                                          & 52.5                                                           & 45.0                                                             & 46.1                                                    \\
                                                     &                                                           &                       &                                                        & 16   & 32.5                                                          & 54.0                                                           & 44.5                                                             & 43.7                                                    \\
                                                     &                                                           &                       &                                                        & 128  & 35.5                                                          & 49.0                                                           & 44.0                                                             & 42.8                                                    \\ \cline{4-9} 
                                                     &                                                           &                       & \multirow{3}{*}{2e-5}                                  & 8    & 32.0                                                          & \textbf{57.0}                                                  & 42.0                                                             & 43.7                                                    \\
                                                     &                                                           &                       &                                                        & 16   & 36.0                                                          & 55.0                                                           & 42.0                                                             & 44.3                                                    \\
                                                     &                                                           &                       &                                                        & 128  & 35.0                                                          & 34.0                                                           & 48.0                                                             & 39.0                                                    \\ \cline{3-9} 
                                                     &                                                           & \multirow{6}{*}{3e-5} & \multirow{3}{*}{1e-4}                                  & 8    & \textbf{56.0}                                                 & 56.5                                                           & 51.5                                                             & \textbf{54.7}                                           \\
                                                     &                                                           &                       &                                                        & 16   & 49.5                                                          & 53.5                                            
               & 52.0                                                             & 51.7                                                    \\
                                                     &                                                           &                       &                                                        & 128  & 44.0                                                          & 49.0                                                           & 44.5                                                             & 45.8                                                    \\ \cline{4-9} 
                                                     &                                                           &                       & \multirow{3}{*}{2e-5}                                  & 8    & 50.0                                                          & 54.0                                                           & 52.5                                                             & 52.2                                                    \\
                                                     &                                                           &                       &                                                        & 16   & 29.0                                                          & 42.0                                                           & 49.5                                                             & 40.2                                                    \\
                                                     &                                                           &                       &                                                        & 128  & 42.0                                                          & 50.0                                                           & 49.5                                                             & 47.2                                                    \\ \cline{2-9} 
                                                     & \multirow{10}{*}{179,727}                                 & \multirow{3}{*}{1e-4} & \multirow{3}{*}{1e-4}                                  & 8    & 34.5                                                          & 43.0                                                           & 46.0                                                             & 41.2                                                    \\
                                                     &                                                           &                       &                                                        & 16   & 27.5                                                          & 40.5                                                           & \textbf{58.5}                                                    & 42.2                                                    \\
                                                     &                                                           &                       &                                                        & 128  & 32.0                                                          & 38.0                                                           & 53.5                                                             & 41.2                                                    \\ \cline{3-9} 
                                                     &                                                           & \multirow{4}{*}{1e-6} & \multirow{2}{*}{1e-3}                                  & 4    & 36.5                                                          & 45.5                                                           & 34.5                                                             & 38.8                                                    \\
                                                     &                                                           &                       &                                                        & 8    & 32.5                                                          & 39.5                                                           & 32.5                                                             & 34.8                                                    \\ \cline{4-9} 
                                                     &                                                           &                       & \multirow{2}{*}{1e-4}                                  & 4    & 35.0                                                          & 45.0                                                           & 47.0                                                             & 42.3                                                    \\
                                                     &                                                           &                       &                                                        & 8    & 30.0                                                          & 43.0                                                           & 32.5                                                             & 35.2                                                    \\ \cline{3-9} 
                                                     &                                                           & \multirow{3}{*}{3e-5} & \multirow{2}{*}{1e-3}                                  & 4    & 28.0                                                          & 40.5                                                           & 50.0                                                             & 39.5                                                    \\
                                                     &                                                           &                       &                                                        & 8    & 31.0                                                          & 38.5                                            
               & 48.5                                                             & 38.2                                                    \\ \cline{4-9} 
                                                     &                                                           &                       & 1e-4                                                   & 4    & 34.0                                                          & 44.0                                                           & 49.0                                                             & 42.3                                                    \\ \hline
13b                                                  & 179,727                                                   & 3e-5                  & 1e-4                                                   & 8    & \textbf{75.0}                                                 & \textbf{71.0}                                                  & \textbf{70.5}                                                    & \textbf{72.17}                                          \\ \hline
\end{tabular}
}
\end{table}


==> tex/09_realworld.tex <==
\input{tex/result_table}
\subsection{Generalization to Real-World Data}

\parlabel{Data Collection}
To test real-world applicability, we collect a new dataset from 10 adult participants using personal smartphones and the Sensor Logger app~\cite{tszheichoiSensorLogger}. Participants, recruited via campus boards and social media, recorded \textit{nine} predefined activities (Table~\ref{tab:opensqa_sources}) in familiar settings—70\% on campus, 30\% at home. Devices included iPhone, Samsung, and Pixel models, capturing diverse hardware conditions.

Each activity lasted ~2 minutes and was performed in a fixed order while holding the phone. This setup introduces natural variability and noise, particularly relevant to the “Reliability” aspect of QA. The dataset, reflecting a range of real-world scenarios, is available in our repository.

\noindent\textbf{Data Processing.}
We discard the first/last 2 seconds of each recording, then split the remaining data into 6-second segments and downsample from 100Hz to 20Hz for consistency. From ~20 segments per activity per user, we sample a few and generate 3 QA pairs (focused on reliability and narration), resulting in 534 total QA examples grounded in user-collected smartphone IMU data.

\parlabel{Evaluation}
We evaluate LLaSA-7b against Vicuna-13b-1.5-16K on 50 randomly chosen QA pairs per category, using the quality metric from Section~\ref{sensor-qa-eval-scoring}. All QAs are derived from real-world smartphone accelerometer and gyroscope readings. To account for sensor and context variability, we prompt GPT-4o to adjust expectations during scoring. As shown in Table~\ref{tab:realword_results}, LLaSA performs comparably or better than on curated PAMAP2 data—demonstrating its robustness to uncontrolled, noisy input and outperforming larger general-purpose models despite a smaller context window and compressed feature input.


==> tex/Experimental_setup.tex <==
\section{Experimental Setup}
\subsection{Experiments}
We conduct a series of experiments to evaluate LLaSA on both open-ended and close-ended QA, fine-tune model parameters, assess model scalability, and validate performance in real-world scenarios.

\noindent\textbf{Open-Ended QA:} We evaluate the model’s ability to generate contextual responses from raw sensor data. Given sensor inputs corresponding to different human activities, the model is prompted with open-ended questions requiring reasoning about the activity context. The objective is to assess the model’s capacity for understanding, inference, and contextual awareness beyond direct classification. For automated evaluation, we utilize 30 QA pairs distributed evenly among the categories. To simplify human evaluation, we pick a subset of 10 QA pairs that represent the range of GPT-assisted scores our model achieved while also ensuring diversity of human activities, sensor locations, and evaluation categories.

\noindent\textbf{Close-Ended QA: } We perform zero-shot classification on raw sensor data for human activity recognition, where zero-shot means that we do not explicitly train the model for classification. The model is prompted with predefined activity categories and asked to classify the given IMU signals accordingly. This experiment assesses the model’s capability to generalize to unseen data and recognize activities without explicit fine-tuning on labeled datasets.

\noindent\textbf{Hyper-parameter Tuning} To optimize model performance for IMU-related question-answering tasks, we fine-tune key hyperparameters, including learning rate, batch size, and sequence length, using our . The goal is to maximize inference quality and efficiency, ensuring that the model effectively processes and responds to IMU-based queries.

\noindent\textbf{Model Scaling: } We investigate the impact of model size on question-answering performance by evaluating different configurations of the model. This experiment explores how larger model variants influence accuracy, response coherence, and computational efficiency, providing insights into the trade-offs between model complexity and performance.

\noindent\textbf{Real-Word Evaluation: } To assess real-world generalization, we collect a new dataset comprising human activity data from participants of diverse backgrounds, performing activities in varied real-world scenarios while carrying a mobile phone. The collected data is used to benchmark our approach against existing baseline models. Performance is evaluated based on both open-ended responses and classification accuracy, providing a comprehensive comparison of model robustness in realistic conditions.

\subsection{Datsets}
We evaluate LLaSA on our proposed OpenSQA dataset for open-ended tasks (details in section \ref{opensqa-dset}) and close-ended tasks were evaluated on $5$ publicly available human activity recognition datasets.

\noindent\textbf{HHAR ~\cite{stisen2015smart}.} The HHAR dataset includes accelerometer and gyroscope recordings from $9$ users performing $6$ activities: biking, sitting, standing, walking, climbing upstairs, and going downstairs. Data was collected using $6$ smartphone models, worn around the waist with sampling rates ranging from $100$ Hz to $200$ Hz.

\noindent\textbf{MostionSense ~\cite{malekzadeh2019mobile}.} ollected using an iPhone 6s, this dataset contains accelerometer and gyroscope time-series data from 24 participants of diverse gender, age, weight, and height. Participants performed 6 activities (walking, jogging, sitting, standing, going upstairs, and going downstairs) with the phone in their front pocket, recorded at 50 Hz.

\noindent\textbf{Shoaib ~\cite{shoaib2014fusion}.} his dataset captures 7 physical activities (walking, sitting, standing, jogging, biking, walking upstairs, and walking downstairs) from 10 male participants. Each participant carried 5 Samsung Galaxy S II smartphones placed at different body positions (right pocket, left pocket, belt, upper arm, and wrist). Data includes accelerometer, gyroscope, and magnetometer readings, recorded at 50 Hz.

\noindent\textbf{UCI ~\cite{reyes2016transition}.} This dataset includes accelerometer and gyroscope data from 30 volunteers (ages 19–48) performing 6 activities (standing, sitting, lying, walking, walking upstairs, and walking downstairs). Data was collected using a Samsung Galaxy S II worn on the waist, with a constant sampling rate of 50 Hz.

\noindent\textbf{SHL ~\cite{gjoreski2018university}.} A large-scale multi-sensor dataset includes various sensor modalities such as accelerometer, gyroscope, orientation, gravity, and GPS. It captures activities like sitting, walking, and running, both in every day and transportation scenarios, such as traveling by bus or train. 

\subsection{Baselines}
\noindent\textbf{Vicuna-7b-16k ~\cite{}} Vicuna 7B-16K is an open-source large language model (LLM) based on Llama 2, designed for efficient and high-quality text generation. It features 7 billion parameters and supports an extended 16K token context window, enabling it to handle longer conversations and documents effectively.

\noindent\textbf{GPT 3.5-T ~\cite{}} GPT-3.5-T is a variant of OpenAI’s GPT-3.5 model, optimized for efficiency and performance in text generation, reasoning, and conversation tasks.  While specific details about its architecture and parameter count may vary, it is designed to handle complex queries, assist in coding, generate high-quality text, and support multi-turn interactions effectively.

\noindent\textbf{GPT-4o-mini ~\cite{}}


\noindent\textbf{GPT-4o ~\cite{}}

\noindent\textbf{GPT 3.5-T-F ~\cite{}}


\subsection{Evaluation Metrics}
For the close-ended task, we report the \textit{F1-Score}, \textit{Precision}, and \textit{Recall} for all baselines alongside LLaSA. Additionally, we provide the context length used by each baseline, highlighting the model complexity required to achieve a given level of zero-shot classification performance.

For open-ended tasks such as comparisons with baseline LLMs, real-world evaluation, and hyperparameter tuning to find the best model capable of following sensor-aware instructions, we compare different model sizes using three key metrics: \textit{Narrative QA Score}, \textit{Reliability QA Score}, and their mean, \textit{Overall Score}, ensuring a fair comparison. The scoring system follows the framework we present in Section \ref{subsec:quality_score}. Additionally, we include qualitative examples to provide deeper insights and enhance understanding of the model's responses.

==> tex/Table_sensorcap.tex <==
\begin{table*}[]
\caption{Prompt design for SensorCaps generation. We prompt GPT-4o-mini with specific instructions to generate a caption for the sensor data in 20-25 words and generate a step-by-step narration of the activity's sensor reading.}
\label{tab:sensorcap_propmt}
\begin{footnotesize}
\resizebox{\linewidth}{!}{
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{CBCEFB}\textbf{Instruction for Generating SensorCaps}}           \\ \hline
\multicolumn{2} {|p{\textwidth}|}{\begin{tabular}[c]{@{}p{\textwidth}@{}}
Please consider yourself to be an expert on gyroscope and accelerometer sensor information given as metadata of IMU datasets. You are given the IMU sensor readings of human activity. The user also provides a brief summary of the event followed by 'Summary:'. They also give you gyroscopic and accelerometer sensor data followed by 'Gyroscope:' and 'Accelerometer:' respectively. They are written in a Python list of lists format and contain x, y, and z-axis data, respectively. Please pay attention to the values and the signs. Additional information computed for each axis is provided afterward, with the windows for moving averages being 12. You should provide comprehensive detail of at least a couple of characteristic IMU features for that event within 20-25 words, followed by 'Features:.' The IMU features should be concise and descriptive. Separate multiple features with commas. Derive the list of features based on the given sensor data. Then, narrate the temporal event with details that are context-aware based on the sensor data, followed by 'Narration:' in a step-by-step fashion, analyzing it within 500 words or less. Please analyze even the small movements thoroughly in a logical and contextual manner, utilizing a deductive thought process while being aware of the knowledge regarding the meaning of the sensor data. Use descriptive terms that aren't vague. \\

\end{tabular}}
\\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{CBCEFB} \textbf{Prompt Input Structure}}   & \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB} \textbf{Output Structure}} \\
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}p{0.5\linewidth}@{}}1. Activity class label \\ 2. Gyroscope sensor data \\ 3. Accelerometer sensor data\\ 4. Sensor location \\ 5. Handcrafted features: moving averages, FFT, min, max, median, variance for each axis\end{tabular}}                                             & \begin{tabular}[c]{@{}l@{}}1. Characteristics IMU features in natural language \\ 2. Narration of the activity's sensor readings\end{tabular}                                                                                                                                                                                                                                                                                                               \\ \hline
\end{tabular}}
\end{footnotesize}
\end{table*}
